Spontaneous Pulse Formation in Edge-Less Photonic Crystal Resonators

Complex systems are a proving ground for fundamental interactions between components and their collective emergent phenomena. Through intricate design, integrated photonics offers intriguing nonlinear interactions that create new patterns of light. In particular, the canonical Kerr-nonlinear resonator becomes unstable with a sufficiently intense traveling-wave excitation, yielding instead a Turing pattern composed of a few interfering waves. These resonators also support the localized soliton pulse as a separate nonlinear stationary state. Kerr solitons are remarkably versatile for applications, but they cannot emerge from constant excitation. Here, we explore an edge-less photonic-crystal resonator (PhCR) that enables spontaneous formation of a soliton pulse in place of the Turing pattern. We design a PhCR in the regime of single-azimuthal-mode engineering to re-balance Kerr-nonlinear frequency shifts in favor of the soliton state, commensurate with how group-velocity dispersion balances nonlinearity. Our experiments establish PhCR solitons as mode-locked pulses by way of ultraprecise optical-frequency measurements, and we characterize their fundamental properties. Our work shows that sub-wavelength nanophotonic design expands the palette for nonlinear engineering of light.

==> notes.tex <==
%\hl{SY: Will try to get the tenses through the paper into this 'simple present' case}
%\hl{In terms of verb tense, please do not write "is dictated." https://www.grammarly.com/blog/verb-tenses/ \\
%Useful link on tenses above.  When I write papers, I use the ''simple present'' tense in describing our work. ``We use the simple present tense when an action is happening right now, or when it happens regularly (or unceasingly, which is why it’s sometimes called present indefinite.)'' In introduction or conclusion remarks, I sometimes use present perfect tense to capture that things have been happening in the past. ``The present perfect tense refers to an action or state that either occurred at an indefinite time in the past (e.g., we have talked before) or began in the past and continued to the present time (e.g., he has grown impatient over the last hour).''
%I don't prefer the ``is directed'' present continuous tense, because this makes an action seem ambiguous.  The action may or may not be the regular state of practice.  For example: ``The VCO is used to make the soliton, but maybe in the future we will do something else.'' versus ``We use the VCO to make a soliton.''}

%%%%%%%%%%%%%%%%%%%%%%%%%% on modes

%\hl{SY: I think the question here is: what is 'comb' frequency vs 'resonator' frequency, at which point is there a distinction, and which one does Kerr shift apply to. Let's say we have a single-mode, loss-less, nonlinear harmonic oscillator. In this system, the field will pick up phase at some frequency depending on its natural frequency and field amplitude, but there is no difference between 'field' (or 'comb') frequency versus 'mode' (or 'resonator') frequency. The differense shows up when the oscillator is driven by an external field F, where F has a defined frequency. Then, the 'field' frequency will always equal to the drive frequency, but we can still ascribe the 'mode' frequency like before. In this case the two can be different, and when they are different, the resonator is 'off-resonance' because the driving field will not optimally transfer energy to the resonator. Instead, it will have a very large imaginary component which drags the resonator onto the driving frequency.}

%\hl{Then ,the next question is which one do we ascribe the Kerr shift to. I've been grouping it to the resonator ('mode'), hence the 'hot-resonator frequency' nomenclature. I think this links pretty well with the $n_2$ reference we had earlier in the manuscript, since $n_2$ infers an actual change to the index of the mode, based on the oscillation amplitude.}

%\hl{SY: I made an illustration in the Supplemental materials that provides the steps (or hierarchy) linking the spatial periodicity $\mu$ to the comb modes. $\mu$ is shared between the 'resonator' mode and 'comb' mode in the way a pendulum is linked to the amplitude it swings at, and I think while we can separate infer the frequency of the 'comb' and 'resonator' components, I don't think they can be separated into two sets of mode order $\mu$'s.}


%%%%%%%%%%%%%%%%
%From the early sections 

%Since spontaneous formation of Turing patterns from break-up of the flat state is such a critical outcome in the LLE, we narrow down the physical conditions that lead to it.

%\hl{Here 'comb modes' are on a evenly spaced grid of frequencies, they represent a stable pulse train, their frequencies are linked and cannot be shifted individually. 'resonator modes' are modes with fixed azimuthal orders, with frequencies controlled by their effective index, including material, geometric, and Kerr-induced index changes. The 'modal detuning' is the difference between the two. Is this picture okay?}
\hl{I don't know what modal detuning means.  I don't think that term is useful.  The problem I have is that the following phrase is not true: "balance of the Kerr frequency shift $\delta_\mu$ of resonator mode number $\mu$ ($\mu=0$ being at the pump laser), and the dispersion $\frac{1}{2} \beta \, \mu^2$" Within the LLE we see the balance of the Kerr shift and dispersion.  However, the LLE is entirely about the comb field $a_\mu$.}

\hl{SY: I think the question here is how do we assign physical meanings for each terms in the LLE, which describes the time evolution for field $a_\mu$. This can be done by first considering a single-mode harmonic oscillator:}

\begin{equation}
\partial_t a = -i \omega' a - \gamma_0  a + F e^{i \omega t}
\end{equation}

\noindent \hl{where $\omega'=\omega_0-g |a|^2$ shows the amplitude dependence of the resonance frequency, resulting from expanding $\omega'=\mu \cdot c/L(n_0+n_2 I)$ to first order in $|I|$. If we take this term out by itself, then it becomes the Kerr term $i g |a|^2 a$. This establishes a connection between the Kerr term and a mode's frequency. The following is the picture I hope to present, from Equ. S6:}

\begin{equation}
\partial_\tau a_\mu = -i\alpha  a_\mu + i\delta_\mu \cdot a_\mu + g_\mu\cdot a_\mu + \delta_{\mu 0} F
\end{equation}

\noindent \hl{The 'mode frequency' is defined by rearranging the Kerr term into the harmonic oscillator form, with natural frequency $\delta_\mu = D_{Int}(\mu) + \delta^{Kerr}_\mu$, and a damping (or gain) term $g_\mu=-1+g_\mu^{Kerr}$. Let me put this in the Supplimental section. We can consider moving some to this section later depending on how it looks.}

%\\ The correspondence for infinitesimal amplitude at the Turing pattern onset is calculated, shown in the optional section in supplimental, but I have not made good theoretical correspondence for the soliton state.\\ There is perhaps some flexibility in where to group the Kerr term into. We can interpret it instead as a 'Kerr pump $F^{Kerr}_\mu$, which will be a complex pump amplitude for each mode. In this picture, the 'mode frequency' will only be $D_{int}(\mu)$. The Bao paper actually interpret the pump amplitude F as a 'pump induced modal shift $Im(F/a_0)$', which I find to be strange intuitively. In the end the mathematical form is the same for all of them.}

%By Fourier transform of an LLE solution, we obtain the field amplitudes ($a_\mu$) that correspond to the comb mode number $\mu$ counted with respect to the pump mode. The Kerr frequency shift for the mode $\mu$ is \( \delta_\mu = 2 N_{Ph}- |a_\mu|^2 \), where \(N_{p} = \sum_\nu |a_{\nu}|^2\) is the total photon number \cite{FactorOfTwoBook}.  Energizing the pump mode to achieve balancing of dispersion and nonlinearity \( \omega_{\pm \mu'} = \frac{1}{2} \beta \mu'^2 - \delta_{\pm\mu'} = - \delta_{\mu=0} \approx \omega_0 \) \hl{Here use convention $\beta$ positive} results in the formation of Turing pattern with periodicity $\mu'$. \hl{SY: Need to decide how much math detail here, how much in the following paragraph} The soliton, in contrast, comprises of many phase-locked modes simultaneously Kerr-shifted onto resonance \cite{Bao2014}. Since the pump mode still receives reduced Kerr shift, the soliton state cannot naturally phase-match to the pump mode on resonance. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%stuff after the here we show paragraph

%is a stationary state composed of many modes oscillating in unison at the same detuning $\alpha_s$, illustrated in Fig. \ref{Fig:Conceptual}B \BLogo{}. The soliton state lives at a large negative detuning of the pump laser, made possible by a combination of self- and cross-phase modulation Kerr-shifting the corresponding modes onto resonance \cite{SelfCrossBook, Bao2014}. The difference in Kerr shift of the $\mu=0$ mode from the $\mu'\neq 0$ modes, \(\xi_{Kerr}\ = \delta_{\mu\neq 0}-\delta_{\mu=0}\), remains in the soliton case. \hl{This difference emerges from LLE calculations} \cite{Bao2014} \hl{, and can be intuitively understood as the difference in effective index -- where the pump mode experiences the average index over the resonator, the modes comprising the soliton see the peak intensity.} The smaller Kerr shift of the $\mu=0$ mode than the soliton detuning needs to be compensated for by the pump field F. Operationally, this is to say the pump laser is far-red-detuned from the hot-cavity pump mode when the soliton state is sustained. The red detuning holds a weak flat state amplitude to preclude the Turing pattern, but also prevents spontaneous generation of soliton pulses from the background.

%\hl{Some duplicated info with previous paragraph, maybe need to merge?} At the onset of the Turing pattern (Fig. \ref{Fig:Conceptual}A), the pump mode Kerr shift, \(\delta_{\mu=0} = 2 N_{Ph}-|a_0|^2= |a_0|^2\), is half as large as that of all other modes \(\delta_{\mu'\neq 0} = 2|a_0|^2\). This differential Kerr shift aids in the energy conservation requirement for four-wave mixing \BLogo{}. This phase-matching condition is illustrated by the dashed horizontal line in Figure \ref{Fig:Conceptual}A, therefore energizing the Turing pattern modes, shown as blue dots. 

%\hl{Regarding the blue dots, they would be the 'comb modes', always tracing the laser detuning modulo FSR, therefore sitting on the dashed line. This lining-up reflects energy conservation if we recall the modal LLE before the rotating-wave approximation. The Kerr term in this picture is $\sum(a_i a^\dag_j a_k exp(i (\omega_i - \omega_j +\omega_k)t))$, where, if the comb modes are evenly spaced, the omega terms cancel. The confusing point here is that if we demand both time-independent amplitude and no extra 'pump' terms on the comb modes, the open circles and the blue dots necessarily line up. We may encounter challenges from reviewers whether the mismatch is a cause of detuned pump field, or the result of detuned pump field.}

% Importantly, at the onset of the Turing pattern, the pump mode $\omega_{\mu=0}$ shift \(\delta_{\mu=0} = 2|a_0|^2-|a_0|^2\) is twice smaller than the remaining $\omega_{\mu\neq 0}$ modes \hl{this must be $\mu \neq 0$ ??} \(\delta_{\mu=0} = 2|a_0|^2\). This differential shift between the pump mode and the remaining modes enables the phase-matching condition for generation of the Turing pattern \BLogo{}, indicated by the dashed horizontal line in Figure \ref{Fig:Conceptual}A. \hl{approximately laser on resonance, FWM condition}

%Train of thoughts: Stationary waveform with all modes --> all modes need to be the same frequency (blue dots line up) --> reason why that mode isn't insane-pump-power is modes can be pulled onto resonance (cite Bao) --> but then there's Kerr mismatch, so pump mode cannot be on resonance.

%\hl{the turing pattern has the proper phase matching for four-wave mixing, and maybe we can say the soliton does not... SY: I think this is right (if, somewhat hard to describe without Fig1 panels). How about the following arguments:\\ To get spontaneous comb, it needs to be near resonance --> it's easy to get the 3 modes into resonance altogether in Turing pattern --> The soliton has many modes, and we need them to be all on resonance --> This won't work because the pump Kerr shift is still smaller, but the dispersion is flattened out by mode-pulling, a special characteristics of solitons --> If the pump light is on resonance with the soliton modes, it is necessarily off-resonance from the hot-cavity pump mode.}

%\hl{Writing this out would be:} In the Turing pattern case, the phase-matching condition can be matched by summing the anomalous dispersion and the differential Kerr shift between $\mu=0$ and $\mu'\neq 0$ modes. In the soliton state, however, the mode-pulling characteristics of this state \cite{Bao2014} forces all $\mu'\neq 0$ modes onto the same detuning. This leaves no remaining dispersion to fill in the differential Kerr shift, therefore placing the soliton existence range far-red-detuned from the hot-cavity pump mode. This is so to say at the onset of the Turing pattern, all modes -- pump, signal, and idler -- can be brought onto simultaneous resonance. In the soliton case, if the balance is achieved for the $\mu'\neq 0$ modes, it is not achieved for the $\mu=0$ mode as a result of the differential Kerr shift.

%\hl{So to say (if we reference to the figure here), in Fig 1A there's the quadratic dispersion curve that moves together under Kerr shift, so there is going to be a pair of crossing somewhere. But in the soliton case where dispersion shifts all non-pump modes onto the shared horizontal line, there is no dispersion curve left-over for the pump frequeny to cross anymore. This way the soliton's property (the mode pulling against dispersion) differentiates it from the Turing rolls (all modes have constant shift). This is to say the larger red detuning of the soliton state from the pump is a result of its detuning structure, instead of its cause.} 

%\hl{PhC explaination paragraph}
%which suppresses scattering to unguided modes given $a < \lambda/2$. A PhC waveguide demonstrates a photonic bandgap \cite{PhCBook}, a frequency range where guided propagating mode exists.  In this work, we instead make use of the property that the bandgap strongly modifies the modes in its vicinity, in an edge-less configuration -- where the PhC waveguide forms a azimuthally uniform ring. %The remaining modes of the ring remain unperturbed, provided that the bandgap is significantly smaller than the ring mode spacing. We precisely control the mode shift by the PhC modulation amplitude. This frequency shift is directly imprinted onto the dispersion profile and robust against perturbation.
%\hl{Do we cite Dan Cole's bidirectional comb generation paper, or do we wait to see if referees complain, and then add it?}
 
%\hl{How far do we interpret the hot-resonator modes? Fundamentally it is a 'phase-per-unit-time' quantity, so it is a true frequency in this aspect. However, I tried briefly to derive a form where the pump mode is F + A exp (i delta t), in hope that the resonator will build up amplitude proportional to A to first order, but that didn't work because there is a counter-rotating term at 2 delta frequency that won't go away. (We cannot use extra rotating-wave approx here unless delta is very large, at which point the shift just sees the average intensity, shifting at $2|psi_s|^2$ as if it were a cross-mode shift.) For now let's just qualify the statement and not over-claim. Additionally, I suspect this 2-delta term has something to do with breather oscillations. Need to look into that.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%stuff regarding fig. 1

%% OLD VERSIONS
%The soliton requires a large negative detuning ($\xi_\text{Kerr}=\alpha_s$ \hl{likely this means we don't need $\xi_{Kerr}$}) of the pump laser, holding a weak flat state amplitude to preclude the Turing pattern. Startlingly, the combination of self- and cross-phase modulation of the soliton waveform \cite{SelfCrossBook, FactorOfTwoBook, Bao2014} pulls all of the XX; see Fig. S2 for a detailed calculation.
%The frequency structure in the DKS case is more complex from a combination of both self- and cross-phase modulation \cite{SelfCrossBook, FactorOfTwoBook}, but a difference in Kerr shift between $\omega_{\mu=0}$ and $\omega_{\mu' \neq0}$ modes remain, shown in Figure \ref{Fig:Conceptual}B. 
%% ENd OLD VERSIONS

%This can be understood intuitively as that the $\omega_{\mu\neq0}$ modes in the DKS live inside the body of the pulse, experiencing higher intensity, and therefore larger Kerr shift. The $\omega_{\mu=0}$ mode exists across the entire resonator and samples the average effective index, resulting in a smaller Kerr shift. I DON'T THINK THIS INTUITIVE PICTURE HELPS ENOUGH COMPARED TO DISTRACTING FROM WHAT'S IN FIG. 1.
%The DKS state exists with the $\omega_{\mu\neq0}$ modes pulled onto resonance \cite{Bao2014} with the pump laser (modulo the cold-cavity mode spacing), but the smaller Kerr shift of the hot-cavity $\omega_{\mu=0}$ mode means it is off-resonance from the pump laser in the same condition. This Kerr-mismatch, denoted as $\xi_{Kerr}$, results in the DKS existing far-red-detuned from the $\omega_{\mu=0}$ mode \BLogo{}. When the resonator is energized at near-resonance detuning from the hot-cavity pump mode, the flat amplitude is high, and becomes unstable against vacuum fluctuation \cite{Godey2014}. The modes that are phase-matched create the Turing pattern, shown in Fig. \ref{Fig:Conceptual}A. If the resonator is energized at the DKS existence detuning instead, the flat amplitude is low and DKS cannot be spontaneously excited. Hence, DKSs must be seeded by Turing-like states or other chaotic states \BLogo{}.

%The existence detuning determines the pattern formation behavior through the stability of the flat-amplitude background against excitation. The Turing pattern can arise because it exists near-resonance and the background is unstable, while the DKS cannot spontaneously form from an empty cavity in its far-red-detuned existence range .

%\hl{this paragraph would be difficult for a non-extreme-expert to understand.  I am modifying it above}
%The dissipative Kerr soliton (DKS) is an optical state composing of a high-intensity pulse coexisting with a flat-amplitude background that is continuously energized. This two-component nature results in the pump ($\mu = 0$) and non-pump ($\mu \neq 0$) modes behaving differently under Kerr shift \cite{FactorOfTwoBook}. Relative Kerr shift between modes phase-match nonlinear effects, such as the Turing pattern formation in Figure \ref{Fig:Conceptual}A. 

%In the DKS, the energy in the non-pump modes is contained inside the pulse, sampling the pulse intensity and a higher effective refractive index. This mechanism enables solitons to exist in significantly larger red detuning from the cold-cavity resonance frequency compared to other states. The pump mode, however, exists across the entire resonator and samples the average effective index, resulting in a smaller Kerr shift. As the non-pump modes shift into near-resonance to the pump light, the pump mode lags behind with its smaller shift. This mismatch in Kerr shift $\xi_{Kerr}$ is shown in Figure \ref{Fig:Conceptual}B. The mismatch results in the pump light being red-detuned from the pump mode in the pulse state. The conventional method to generate the DKS is sweeping the pump light blue-to-red across the pump mode. The resonator undergoes the Turing rolls with number determined by dispersion, followed by a chaotic state where pulses form and disappear sporadically \cite{Bao2014}, then arrives at the red detuning where pulses from the chaotic state stabilize into the DKS. The number of pulses formed this way is not deterministic. This is also not spontaneous in that the resonator will remain empty if the DKS is lost.

